WTS: A Pedestrian-Centric Traffic Video Dataset for Fine-grained Spatial-Temporal Understanding

In this paper, we address the challenge of fine-grained video event understanding in traffic scenarios, vital for autonomous driving and safety. Traditional datasets focus on driver or vehicle behavior, often neglecting pedestrian perspectives. To fill this gap, we introduce the WTS dataset, highlighting detailed behaviors of both vehicles and pedestrians across over 1.2k video events in hundreds of traffic scenarios. WTS integrates diverse perspectives from vehicle ego and fixed overhead cameras in a vehicle-infrastructure cooperative environment, enriched with comprehensive textual descriptions and unique 3D Gaze data for a synchronized 2D/3D view, focusing on pedestrian analysis. We also pro-vide annotations for 5k publicly sourced pedestrian-related traffic videos. Additionally, we introduce LLMScorer, an LLM-based evaluation metric to align inference captions with ground truth. Using WTS, we establish a benchmark for dense video-to-text tasks, exploring state-of-the-art Vision-Language Models with an instance-aware VideoLLM method as a baseline. WTS aims to advance fine-grained video event understanding, enhancing traffic safety and autonomous driving development.

==> sec/7_localization.tex <==
%% I moved this part to section3.3 3D Location part
\section{Localization (TO BE MOVED SOMEWHERE ELSE)}
\label{sec:localization}

To localize the subjects (person and vehicle) in the virtual environment, we employ the following pipeline as shown in fig. (TODO: REF. FIGURE?) to estimate the yaw and pitch of the subjects from camera sensor. The pipeline encompasses the following blocks:

\textbf{Object Detection and Tracking}
We use Yolov8x \cite{Alpher05} for object detection. Yolov8x has 67.2M parameters and 257.8B FLOPs. Yolov8x model supports the tracking. We use Bytetrack \cite{zhang2022bytetrack} to track the bounding boxes across the frames. 

\textbf{Pitch and Yaw estimation}
To estimate the location of the subjects with respect to camera sensor we first estimate the yaw and pitch angle of the subject. Let's assume K represents the camera matrix, then we use the following to calculate the direction vector ($d$) extending from the optical center to image point.

\begin{equation}
d = K^{-1} \cdot p
\end{equation}

From direction vector $d$, we can calculate the yaw and pitch as following

\begin{equation}
yaw = \arctan(\frac{{d_x}}{{d_y}})
\end{equation}

\begin{equation}
pitch = \arctan(\frac{{d_y}}{{d_z}})
\end{equation}


\textbf{3D localization}
 For 3D localization, we align the cameras within the virtual world using the camera extrinsic parameters such as pose. Our approach to estimate the distance of the subjects involves the estimating the ray vector from the camera's sensor, directed by the yaw and pitch angle (ffrom previous step) until it intersects the plane (z=0) within the virtual environment. The resulting intersection point is the location of corresponding subject. Finally we use the blender environment to render the image.


